Beyond Anonymization: Object Scrubbing for Privacy-Preserving 2D and 3D Vision Tasks

We introduce ROAR (Robust Object Removal and Re-annotation), a scalable framework for privacy-preserving dataset obfuscation that eliminates sensitive objects instead of modifying them. Our method integrates instance segmentation with generative inpainting to remove identifiable entities while preserving scene integrity. Extensive evaluations on 2D COCO-based object detection show that ROAR achieves 87.5% of the baseline detection average precision (AP), whereas image dropping achieves only 74.2% of the baseline AP, highlighting the advantage of scrubbing in preserving dataset utility. The degradation is even more severe for small objects due to occlusion and loss of fine-grained details. Furthermore, in NeRF-based 3D reconstruction, our method incurs a PSNR loss of at most 1.66 dB while maintaining SSIM and improving LPIPS, demonstrating superior perceptual quality. Our findings establish object removal as an effective privacy framework, achieving strong privacy guarantees with minimal performance trade-offs. The results highlight key challenges in generative inpainting, occlusion-robust segmentation, and task-specific scrubbing, setting the foundation for future advancements in privacy-preserving vision systems.

==> figures/labeling_figure.tex <==

\begin{figure}
    \centering
\begin{tikzpicture}[scale=0.45, transform shape,node distance=1.5cm, every node/.style={fill=white, font=\sffamily}, align=center]
  % Nodes specification
  \node (start) [activityStarts] {Labeling Scrubbed Dataset};
  \node (scrubbedImage) [process, below of=start, yshift=-1cm] {Scrubbed Image};

  \node (detectIntersecting) [process, below of=scrubbedImage, yshift=-1cm] {Find (non)-intersecting objects};

  \node (intersectCheck) [base, shape=diamond, aspect=2, below of=detectIntersecting, yshift=-1cm] {Do they intersect?};
   
  % Run Oracle Model
  \node (oracleModel) [process, below of=intersectCheck, yshift=-1cm] {Run Oracle Model: Detect non-person objects};
  
  % Decision for object accuracy
  \node (accuracyCheck) [base, shape=diamond, aspect=2, below of=oracleModel, yshift=-1cm] {Object accuracy $\geq$ \textbf{0.45}?};

  % Annotate object
  \node (annotateObject) [process, right of=accuracyCheck, xshift=4cm] {Annotate object};

  % Skip object
  \node (skipObject) [process, left of=accuracyCheck, xshift=-4cm] {Skip object};

  % All objects skipped?
  \node (allSkipped) [base, shape=diamond, aspect=2, below of=skipObject, yshift=-1cm] {All objects skipped?};
  
  % Delete image if all objects are skipped
  \node (deleteImage) [sensitiveObject, below of=allSkipped,yshift=-1.3cm] {Delete image from dataset};

  % Unlabeled Dataset
  \node (unlabeledDataset) [scrubbedAsk, below of=annotateObject, yshift=-3cm] {Add to the Labeled Train Dataset};




  % Arrows between nodes
  \draw[->] (start) -- node[text width=6cm] {Scrubbed images ready for labeling} (scrubbedImage);
  \draw[->] (scrubbedImage) -- node[text width=8cm] {Find objects that intersect with any person}(detectIntersecting);
  \draw[->] (oracleModel) -- (accuracyCheck);
  \draw[->] (detectIntersecting) -- (intersectCheck);
  
  % Decision branches for accuracy
  \draw[->] (accuracyCheck) -- node {Yes} (annotateObject);
  \draw[->] (accuracyCheck) -- node {No} (skipObject);

  \draw[->] (intersectCheck) -- node {Yes} (oracleModel);
  \draw[->] (intersectCheck.east) -| node {No} (unlabeledDataset.east);
  
  % Loop to check all objects in scrubbed image
  \draw[->] (skipObject) -- (allSkipped);
  \draw[->] (allSkipped) -- node {Yes} (deleteImage);
  \draw[->] (allSkipped.west) |- (oracleModel);
  
  % Continue the process if annotation
  \draw[->] (annotateObject) -- (unlabeledDataset);

\end{tikzpicture}

    \caption{Labeling Scrubbed Dataset}
    \label{fig:v4+_label}
\end{figure}

